Extracting Syntactic Patterns from Databases

Many database columns contain string or numerical data that conforms to a pattern, such as phone numbers, dates, addresses, product identifiers, and employee ids. These patterns are useful in a number of data processing applications, including understanding what a specific field represents when field names are ambiguous, identifying outlier values, and finding similar fields across data sets. One way to express such patterns would be to learn regular expressions for each field in the database. Unfortunately, exist- ing techniques on regular expression learning are slow, taking hundreds of seconds for columns of just a few thousand values. In contrast, we develop XSystem, an efficient method to learn patterns over database columns in significantly less time. We show that these patterns can not only be built quickly, but are expressive enough to capture a number of key applications, including detecting outliers, measuring column similarity, and assigning semantic labels to columns (based on a library of regular expressions). We evaluate these applications with datasets that range from chemical databases (based on a collaboration with a pharmaceutical company), our university data warehouse, and open data from MassData.gov.

==> sections/1-app-scenarios.tex <==
\subsection{Application Scenarios}
In order to demonstrate its applicability, we have identified three applications 
of \sys while working with collaborators in the pharmaceutial industry, 
telecommunications and data integration domain as part of a larger project we 
are building in our group. We introduce these applications, along with the challenges they present.

\subsubsection{Summarization and Attribute Comparison}

% why people want to compare columns
Once some interesting attributes are identified, data analysts often wish to
find other similar attributes, \eg given an attribute ID for a table, find other
similar ones to obtain candidates for joining the datasets together. One option
to achieve this is to compare all attribute values one by one, which is
expensive. 

% how do people do this today
When analysts want to perform this operation today, they use the exact
set-similarity join operation \cite{setjoin1, setjoin2}, which identifies
similar attributes according to a similarity metric such as Jaccard
distance. Another option is to rely on approximate methods, that are cheaper
to compute at the cost of some errors. Approximate methods rely on signatures of the
data, such as minhash \cite{minhash}, and use locality sensitive hashing
\cite{lsh}, modeling the problem as an approximate nearest neighbors one.

\begin{figure}[t]
\centering
\includegraphics[width=0.8\columnwidth]{img/structured_attributes.pdf}
\caption{Example relation with learned Xtructure for its attributes}
\label{fig:examplerelation}
\end{figure}

One complementary approach to the exact and approximate set-similarity method is
to instead learn syntactical representations $X_1, X_2 \in R$ of the attributes, 
and then to compare them with some similarity metric. This requires a similarity function, 
but has the added benefits of being much more efficient for large datasets, and 
being extremely human-readable, potentially allowing for human-in-the-loop interactions. 
Furthermore, the representation need only be learned once, and is useful for 
other applications as well.

% example of real use case
For example, in the context of the Chembl \cite{Gaulton2012ChEMBL} public
chemical database, multiple entities follow a clear syntactical pattern, such as
the attribute \emph{CHEMBL} shown in \F\ref{fig:examplerelation}. Other
attributes in the database that also contain Chembl IDs may not overlap with the
attribute of the table, as their Jaccard distance may be high, however, they are
syntactically similar and still of interest for analysts. The syntactical
similarity can be captured by a representation of the syntactical patterns that
can be compared. This has the benefit for the user that attributes with distinct
values but similar SPRs will be presented as similar, allowing to further explore
entities associated to such IDs.

% enumerate challenges this problem introduces
To be useful for summarization and comparison, an approach that learns
syntactic patterns from attributes, such as \sys, must produce a SPR that is
\textbf{readable by humans}, similar to regexes of common programing languages,
and that is \textbf{comparable to other SPR}, to permit finding similar content.

\subsubsection{Automatic Label Assignment}

% why this is good
Identifying important entities in enterprise settings is one of the fundamental
tasks of data analysts. Having such information helps with semantic search, identify
content that refers to similar concepts, and helps users to understand complex
schemas, among others. 

% how people do this today
Despite the importance of such task, the process is fundamentally manual, which
hampers or precludes its execution in large enterprises. The typical approach is
developers or data stewards annotating with labels the attributes in the
database -- a time consuming and error-prone process. 

% how summaries help here
We have identified one opportunity to automatically label attributes of interest
that have well defined syntactical patterns. Data stewards can write regular
expressions that describe entities of interest and associate a meaningful label
to that regex, producing a library of (regex, label). We can then
learn the SPR of attributes and compare them with the regular
expressions until we find a good match, in which case we can annotate the
attribute with the label associated to the matching regex. Having the SPRs
readily available facilitates comparing with new (regex, label) pairs that are
dynamically added to the library, for example, when a new
entity format is introduced from an external dataset.

% real world example
To understand the usefulness of the approach, consider the example in
\F~\ref{fig:compoundids}. All the attributes are identifiers of compound IDs,
commonly used in the biopharma industry. There is a correspondence between IDs
in each format. However, given an attribute SMILES that refers to compound IDs, it is
impossible to find the corresponding InchiKey attribute: neither the attribute
name, nor the content are similar. Suppose, however, that the
domain-expert -- who knows well the different formats of compounds IDs -- writes a
regular expression for InchiKey numbers and another one for SMILES and add these
regular expressions with the label \emph{compoundId} to a registry or database.
We can then learn the SPR from both attributes using \sys,
comparing with the regexes in the registry and associating the attribute with
the labels of the matching regexes. This would associate the label
\emph{compoundId} with both the SMILES and Inchi attribute, therefore making
them searchable by that semantic label. 

% challenges here
Hence the second challenge and design requirement of \sys is that the SPR it
learns \textbf{must be comparable to those represented by traditional regexes}.
Comparing SPRs to each other is not only useful to find \emph{syntactically
similar content}, but also is a stepping stone in finding \emph{semantically
similar content} in a pseudo-automatic way.

\subsubsection{Syntax-Based Outlier Detection}

% why this is good
One long-standing problem in data management is concerned with data quality. In
the wild, data is dirty: sometimes due to input data errors, such as when human
operators have the responsibility of digitalizing information of the analog
world. Other times, automatically captured data contains errors, too, such as
when a sensor is not properly calibrated or there is a temporal glitch in the
system. There are many types of errors, and no single tool capable of adressing
all of them \cite{errors}.

% how people do this today
Among the different tools used to improve data quality, outlier detectors are
popular \cite{outlier, dboost}. Not all outliers are errors, and not all errors
can be detected through outlier-detectors, but many outliers can indicate that
something is off. This is of particular interest when operating on the key
attributes of datasets that need to be joined together.

% how summaries help here
We observe that by learning the syntactical pattern of an attribute, we can 
detect \textbf{syntax-based outliers}, \ie elements that do not fit well with the
learned SPR. When developers are interested in a specific
attribute, they can feed the values back into the learned SPR, that will
compute a \emph{match score}, interpreted as the fitness of the value in the
SPR, and will tag elements that are beyond a threshold.

% example
Consider the example of \F\ref{fig:examplerelation}, with real ZIP codes from
Boston. The 4th cell value has an issue, the ZIP code is erroneous. In this
case, it is possible to detect it as it has a different lenght than the other
records in the same attribute. In other cases, outliers are not erros. In this
scenario, the 4th cell will be tagged as an outlier: its syntactical pattern is
different from the rest of cells of the attribute.

% challenges
To be able to detect syntax-based outliers, \sys must support the concept of a
\textbf{scoring fit}, \ie how well a particular value fits the learned SPR.
For \sys to be used as an outlier detector, it must not overfit the SPR to
\emph{all} the values, or it will not detect outliers. Instead, it must
represent the general syntactical structure. The details of this are explained
in section \ref{sec:approach}.


==> sections/relatedwork.tex <==
\section{Related Work}

\mypar{Structuring unstructured data}
semantic web

opencalais

\mypar{Semantic web}
rdf and ontologies. this is usually domain specific


links to check

http://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.95.5369&rep=rep1&type=pdf

https://people.cs.umass.edu/~mccallum/papers/mccallum-conll2003.pdf

http://www.cs.huji.ac.il/~arir/concept_specific_relships.pdf

https://homes.cs.washington.edu/~etzioni/papers/knowitall-aij.pdf

http://www.aclweb.org/anthology/D09-1098

http://www.cs.cmu.edu/~./wcohen/postscript/icdm-2007.pdf

http://www.cs.cmu.edu/~./wcohen/postscript/icdm-2008-iseal.pdf

http://www.cidrdb.org/cidr2015/Papers/CIDR15_Paper21.pdf

http://www.cidrdb.org/cidr2015/Slides/10_CIDR15_Slides_Paper10.pdf

http://www.cidrdb.org/cidr2015/Papers/CIDR15_Paper32.pdf

http://dl.acm.org/citation.cfm?id=2467706

SIGIR

http://maroo.cs.umass.edu/pub/web/getpdf.php?id=1143

Learning regex on dirty data

http://delivery.acm.org.libproxy.mit.edu/10.1145/2790000/2786983/a13-bartoli.pdf?ip=18.9.61.112&id=2786983&acc=ACTIVE%20SERVICE&key=7777116298C9657D%2EDE5F786C30E1A3B4%2E4D4702B0C3E38B35%2E4D4702B0C3E38B35&CFID=759690908&CFTOKEN=20307549&__acm__=1457377658_6305ca26aba7691629f37bf399ca9524

